Guess, SWAP, Repeat : Capturing Quantum Snapshots in Classical Memory

We introduce a novel technique that enables observation of quantum states without direct measurement, preserving them for reuse. Our method allows multiple quantum states to be observed at different points within a single circuit, one at a time, and saved into classical memory without destruction. These saved states can be accessed on demand by downstream applications, introducing a dynamic and programmable notion of quantum memory that supports modular, non-destructive quantum workflows. We propose a hardware-agnostic, machine learning-driven framework to capture non-destructive estimates, or "snapshots," of quantum states at arbitrary points within a circuit, enabling classical storage and later reconstruction, similar to memory operations in classical computing. This capability is essential for debugging, introspection, and persistent memory in quantum systems, yet remains difficult due to the no-cloning theorem and destructive measurements. Our guess-and-check approach uses fidelity estimation via the SWAP test to guide state reconstruction. We explore both gradient-based deep neural networks and gradient-free evolutionary strategies to estimate quantum states using only fidelity as the learning signal. We demonstrate a key component of our framework on IBM quantum hardware, achieving high-fidelity (approximately 1.0) reconstructions for Hadamard and other known states. In simulation, our models achieve an average fidelity of 0.999 across 100 random quantum states. This provides a pathway toward non-volatile quantum memory, enabling long-term storage and reuse of quantum information, and laying groundwork for future quantum memory architectures.

==> Abstract_memory_bank.tex <==
One of the central challenges in quantum computing arises from wavefunction collapse during measurement. To determine a quantum state, traditional methods such as Quantum State Tomography (QST) require a series of destructive measurements on multiple copies of the state, ultimately erasing the very state we seek to understand. In this work, we introduce a novel \texttt{Quantum Memory Bank Architecture} that enables the observation of quantum states without directly measuring, and thereby destroying them. 
% 
Our architecture enables the observation of multiple quantum states at different points within a single circuit, allowing them to be saved \texttt{(`deposited')} into a classical memory without direct measurement or destruction. These states can then be accessed \texttt{(`withdrawn')} on demand by downstream applications during execution, introducing a dynamic and programmable notion of quantum memory that supports modular, non-destructive quantum workflows.

We leverage the SWAP test to compute fidelity between an unknown state and a generated estimate to guide both gradient-based and gradient-free optimization strategies to recover the state vector or density matrix from a single copy of the unknown state, using mid-circuit measurement techniques.
% 
A neural network is trained to generate high-fidelity approximations of the unknown state by observing only the ancilla qubit from the SWAP test. It learns to associate changes in its inputs with resulting fidelity scores, allowing it to converge on the correct state. We use state vector and unitary-based techniques to reconstruct pure states, and extend the method to mixed states using density matrix formalism.
% 
Our approach achieves fidelity $\sim 1.0$ for Hadamard states on real IBM superconducting qubit hardware, and an average fidelity of $0.999$ across 1000 random states in simulation. The architecture is hardware-agnostic and applicable to any quantum computing platform. Unlike traditional QST methods, our approach allows single-copy, mid-circuit recovery of quantum states with fidelity $\sim 1.0$ using hardware-validated techniques.
%The codebase is available here \url{https://github.com/DebarshiKunduPSU/NMQST}.    


% Traditional Quantum state tomography (QST) is the process of obtaining a complete description of a quantum system by performing measurements on a set of informationally complete observables and in the process destroying (due to measurement) the original unknown states. 
% We propose a Quantum State Tomography (QST) method without measuring (destroying) the original unknown state using both gradient-based and gradient-free methods for estimating the state vector and density matrix of an unknown quantum state. Our approach leverages the SWAP test to compute fidelity and uses this information to guide the estimation process. By performing multiple SWAP tests within the decoherence time of the unknown state's qubits, our method enables quantum state tomography using only a single copy of the unknown state. 
% We employ a neural network model that iteratively learns to generate the correct state vector or density matrix by measuring only the ancilla qubit. The network learns to associate changes in the input with changes in fidelity, allowing it to generate states with high fidelity. Our method achieves fidelity 1 on real quantum hardware for Hadamard states, and an average fidelity of 0.999 for 1000 random states in simulation.

% This approach introduces a novel paradigm in QST that does not require target unknown states to be measured/destroyed and able to dynamically estimate the unknown state. This opens up new possibilities for algorithm development in dynamic circuits.  The process is hardware-agnostic and feasible for implementation on any quantum computing platform. We demonstrate our results using IBM’s superconducting qubit-based quantum computers. We also demonstrate our method leads to quantum memory because it enables dynamically estimating states and therefore saving the snapshots classically which can be retrieved anytime using quantum memory during dynamic circuit execution. 
% The codebase is available here \url{https://github.com/DebarshiKunduPSU/NMQST}

% Quantum state tomography (QST) is the process of obtaining a complete description of a quantum system by performing measurements on a set of informationally complete observables. However, traditional QST methods require an exponential number of measurements as the system size increases, making them impractical for large-scale quantum systems. QST involves estimating the density matrix of an unknown quantum state through repeated measurements, assuming that the source consistently produces identical copies of the state. 
% However, the assumption of access to multiple identical copies is often unrealistic, particularly in the NISQ (Noisy Intermediate-Scale Quantum) era. 
% In this work, we propose \hl{I think you should start with NN model that is trained using swap test. Right now its all mixed up-- both gradient-based and gradient-free methods for estimating the state vector and density matrix of an unknown quantum state without destroying the original state. Our approach leverages the SWAP test to compute fidelity and uses this information to guide the estimation process. By performing multiple SWAP tests within the decoherence time of the unknown state's qubits, our method enables quantum state tomography using only a single copy of the unknown state. 

% We employ a neural network model that iteratively learns to generate the correct state vector or density matrix by measuring only the ancilla qubit. The network learns to associate changes in the input with changes in fidelity, allowing it to generate states with high fidelity. Our method achieves fidelity 1 on real quantum hardware for Bell states, and an average fidelity of 0.999 for 1000 random states in simulation.

% This approach introduces a novel paradigm in QST that is hardware-agnostic and feasible for implementation on any quantum computing platform. We demonstrate our results using IBM’s superconducting qubit-based quantum computers, which were freely accessible for this work.}

%version 2
% Quantum mechanics imposes a fundamental limitation on observing a system without disturbing its state, complicating the study and control of quantum systems. While quantum state tomography provides a method for reconstructing states through repeated measurements, its destructive nature makes it impractical for larger quantum systems. In this work, we explore a novel approach to reconstruct unknown quantum states using classical machine learning techniques. We propose three primary methods: the first estimates the state using a state vector, the second utilizes a unitary representation, and the third employs a density matrix, with the latter capable of reconstructing both pure and mixed states. Each method leverages a classical neural network to achieve accurate state estimation. \hl{need to add results}
% Although our approach requires classical resources that scale exponentially with the number of qubits ($2^n$ complexity) — a well-known challenge in state reconstruction — this remains feasible for the small-scale circuits typical of the NISQ (Noisy Intermediate-Scale Quantum) era. 



% version 1
% Until more efficient quantum information storage techniques are developed, our method offers a practical solution for near-term quantum memory applications, providing a non-invasive means of accessing state information without direct measurement.

% Can we store Quantum State information classically? We answer the question in this work. We propose a method to figure out an unknown Quantum State with a classical machine learning approach. Although the proposed method needs $2^n$ complexity of classical resources to store quantum state (unsurprisingly ), we have shown this approach is suitable for NISQ era small Qubits until a better method to store quantum information is figured out. 

==> Introduction_memory_bank.tex <==
\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{fig/quantum_bank.pdf}
    \caption{
    \textbf{The Quantum Memory Bank Architecture:}
    Quantum states observed at various points within a circuit are reconstructed and stored in classical memory, without collapsing the original system. This enables non-destructive access to quantum information during circuit execution. Once stored, these reconstructed states can be accessed later by downstream quantum applications that require the reuse or reinitialization of specific states, such as those relying on QRAM-style retrieval. We refer to this process of storing quantum states as state `deposition', and the later retrieval as state `withdrawal'. This architecture supports modular and adaptive quantum workflows, while laying the foundation for classical storage and programmatic reuse of quantum information.
}
    \label{fig:quantum_bank}
\end{figure}

The ability to observe and understand the state of a quantum system lies at the heart of quantum computation, communication, and control. Yet, this seemingly fundamental task is fraught with paradox. In contrast to classical systems, where the act of observation simply reveals information, quantum systems suffer from a unique fragility: the very act of measurement irreversibly alters the state being observed. This phenomenon, known as wavefunction collapse, implies that once a quantum state is measured, it no longer exists in its original form. Consequently, direct measurement not only extracts partial information but also destroys the delicate superpositions and entanglements that are central to quantum advantage. 
%This presents a profound limitation: to know the state is to lose it. 
% As such, any method that seeks to observe a quantum state without collapsing it must walk a fine line between interaction and preservation, offering a pathway toward more intelligent, adaptive, and non-destructive quantum technologies. 
Traditionally, Quantum State Tomography (QST) has been the primary technique for reconstructing a full description of a quantum state, typically represented as a density matrix, by performing repeated measurements on many identically prepared copies. QST is instrumental in verifying prepared states, benchmarking quantum hardware, and characterizing noise in quantum processes, and has become a standard tool for experimental validation. However, it remains fundamentally destructive, as it relies on projective measurements that collapse the quantum state.

\begin{figure*}[]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/process.pdf}
    \caption{
    \textbf{Methodology for Non-Destructive Quantum State Observation:}
    This figure illustrates the methodology behind the three primary processes for observing a quantum state with $n$ qubits, without destroying it. The approach begins with an unknown target circuit (marked in light blue) and a neural network model that generates an output representing either a state vector (Method 1), a unitary (Method 2), or a density matrix (Method 3). This output is used to construct a reconstructed circuit (marked in light purple).  
    An ancilla qubit is initialized in the state \( |0\rangle \), and a swap test is performed between the target and reconstructed circuits. The outcome is projected onto the ancilla qubit, and its measurement yields the fidelity — a measure of similarity between the two states. A fidelity of 1 indicates a perfect match between the reconstructed and target states. If the fidelity is not sufficiently close to 1, the neural network’s model weights are updated using the fidelity value. This iterative process continues until the fidelity converges to a value very close to 1, ensuring accurate state reconstruction.
}
    \label{fig:process}
\end{figure*}

\subsection{Motivation}

Despite its foundational role, QST faces critical limitations that constrain its scalability and real-time applicability. Chief among these is the exponential growth in the number of measurements required with increasing system size.
%, making QST infeasible for large or highly entangled systems. 
More fundamentally, QST is inherently destructive: each measurement collapses the quantum state, requiring many identically prepared copies to reconstruct the original. This is especially problematic in adaptive, interactive, or decision-based quantum algorithms, where intermediate quantum states carry context-dependent information and cannot be discarded or recreated at will. In such settings, conventional QST is not merely inefficient, it is incompatible. This calls for new methods of quantum state observation that preserve coherence, operate within the system’s decoherence window, and enable dynamic interaction with evolving quantum information.
% 
This motivates a growing demand for non-destructive or minimally invasive state characterization techniques, especially those compatible with Noisy Intermediate-Scale Quantum (NISQ) devices. Ideally, such techniques would enable \textit{in-situ} debugging and dynamic analysis of quantum programs without disrupting computation, thereby expanding the scope of QST in practical quantum applications.

Recent years have seen the emergence of deep learning-based approaches to QST~\cite{liu_variational_2020, ahmed_quantum_2021, gaikwad_gradient-descent_2025, quek_adaptive_2018, luu_universal_2024, lange_adaptive_2023}. However, these methods exhibit significant shortcomings. Most are trained and validated using pre-constructed datasets, without providing mechanisms to verify whether the generated state genuinely overlaps with an unknown state encountered in real execution. The models are probabilistic in nature and rely on measurements from multiple identical copies, without offering a procedure to validate the reconstructed state against a live, unknown quantum state.
% 
Moreover, none of these works demonstrate their applicability on real or noisy quantum hardware. This raises critical questions about their practical utility. For example, \cite{gaikwad_gradient-descent_2025} uses the Uhlmann–Jozsa (UJ) fidelity as a loss function, assuming access to the density matrix of the unknown quantum state. But, such access is inherently unavailable; indeed, the very motivation behind QST is the absence of this knowledge. Thus, using UJ fidelity is not just impractical, it is infeasible to compute or implement on quantum hardware. Table~\ref{tab:background_comparison} systematically evaluates the Quantum Memory Bank Architecture alongside established quantum state reconstruction and tomography techniques.

Quantum memory remains a major bottleneck in quantum computing, as current qubit technologies suffer from short coherence times and quantum measurements irreversibly collapse state superpositions~\cite{decoherence_review, quantum_memory_limitations}. Practical quantum memories, though highly desirable for applications such as quantum repeaters, distributed quantum computing, and quantum internet~\cite{kimble_quantum_2008, sangouard_quantum_2011, wehner_quantum_2018}, remain technologically elusive. Given these limitations, a natural question arises: \textit{Can quantum information be extracted and stored classically, without collapsing the state, such that quantum applications can access it later during computation?}


\subsection{Contribution}

\begin{table*}[t!]
\centering
\fontsize{8.0pt}{9.5pt}\selectfont
\caption{Comparative Evaluation of the Quantum Memory Bank Architecture (QMBA) and Prior Quantum State Reconstruction Methods}
\begin{tabular}{cl||c|ccccc}
\multicolumn{2}{c||}{\textbf{Metric}}                                                                                                            & \textbf{QMBA} & \textbf{Liu, et al~\cite{liu_variational_2020}} & \textbf{Ahmed, et al~\cite{ahmed_quantum_2021}} & \textbf{Quek, et al~\cite{quek_adaptive_2018}} & \textbf{Luu, et al~\cite{luu_universal_2024}} & \textbf{Lange, et al~\cite{lange_adaptive_2023}} \\ \hline \hline
\multicolumn{2}{c||}{\textbf{State Preservation}}                                                                                                & \ding{51}            & \ding{55}                           & \ding{55}                             & \ding{55}                            & \ding{55}                           & \ding{55}                             \\ \hline
\multicolumn{2}{c||}{\textbf{Hardware Agnostic}}                                                                                                 & \ding{51}            & \ding{51}                           & \ding{55}                             & \ding{51}                            & \ding{55}                           & \ding{55}                             \\ \hline
\multicolumn{2}{c||}{\textbf{Dataset Requirement}}                                                                                               & \ding{55}            & \ding{55}                           & \ding{51}                             & \ding{51}                            & \ding{51}                           & \ding{51}                             \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Noiseless\\ Simulation\end{tabular}}}} & \textbf{Min. Fidelity Achieved} & $0.999$        & $0.991$                       & $0.9$                           & $0.999$                        & $0.97$                        & $0.956$                         \\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                         & \textbf{\# Training Epochs}              & $39$           & $240$                         & $1000$                          & \texttt{NA}                           & $1300$                        & $1000$                          \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Noisy\\ Simulation\end{tabular}}}}     & \textbf{Min. Fidelity Achieved} & $0.99$         & \ding{55}                        & \ding{55}                             & \ding{55}                            & $0.3$                         & $0.9093$                        \\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                         & \textbf{\# Training Epochs}              & $xyz$          & \ding{55}                         & \ding{55}                             & \ding{55}                            & $1300$                        & $1000$                          \\ \hline
\multicolumn{2}{c||}{\textbf{Quantum Hardware Result}}                                                                                                   & \ding{51}            & \ding{55}                           & \ding{55}                             & \ding{55}                            & \ding{55}                           & \ding{55}                             \\ \hline \hline
\end{tabular}
\label{tab:background_comparison}
\end{table*}

In this work, we propose a novel Quantum Memory Bank Architecture for dynamic quantum state observation using mid-circuit measurements, enabling state reconstruction during the execution of a quantum circuit. Crucially, this is achieved without collapsing or destroying the quantum state, allowing multiple states at multiple points within the circuit to be accessed and stored. Our method estimates the quantum state and saves it into classical memory, a process we term state \texttt{`deposition'}. These stored (or deposited) states can later be retrieved or re-prepared by downstream applications as needed, a process we call state \texttt{`withdrawal'}. 
% 
This approach has broader implications, particularly for the classical storage and reuse of quantum information. By reconstructing and storing quantum states as classical vectors, our method lays the foundation for a form of classical quantum memory. These reconstructed states can be reloaded (`withdrawn') by quantum applications requiring access to previously encountered states, such as those employing standard QRAM retrieval algorithms, thus enabling non-destructive reuse without relying on persistent physical quantum memory.
 
Fig.~\ref{fig:quantum_bank} provides an overview of the Quantum Memory Bank Architecture, while Fig.~\ref{fig:process} illustrates the detailed methodology for non-destructive quantum state observation. Although this work focuses primarily on state `deposition', we also discuss select use cases where state `withdrawal' enables modular and adaptive quantum workflows.
 
The primary contributions of this paper are as follows:
% 
    \textbf{(1) Mid-circuit quantum state reconstruction:} We propose a technique for performing quantum state tomography dynamically during circuit execution using mid-circuit measurements. This enables non-destructive monitoring and debugging of quantum programs, even within adaptive quantum algorithms.
% 
    \textbf{(2) Neural network-guided state generation:} We use a classical neural network to generate candidate quantum states that approximate an unknown target state. These candidates are prepared on quantum hardware using the Möttönen state preparation technique~\cite{mottonen_transformation_2004}, implemented via \texttt{qml.StatePrep}~\cite{noauthor_qmlstateprep_nodate}. The network’s output defines the parameters for constructing state preparation circuits based on the Möttönen decomposition, enabling precise initialization of quantum states during training.
% 
    \textbf{(3) Fidelity estimation via SWAP test:} We perform a SWAP test between the unknown quantum state and a generated candidate using mid-circuit measurements (detailed in Section~\ref{methods}) to estimate their overlap. The outcome of the SWAP test, a fidelity score, serves as a feedback signal for a neural network trained to generate quantum states that closely approximate the unknown target. By iteratively generating candidate states and comparing them to the unknown state via the SWAP test, the network gradually reconstructs the original quantum state, up to a global phase, which is irrelevant for most quantum computing applications (see page 15 in \cite{Nielsen_Chuang_2010}). This fidelity-driven learning loop enables high-accuracy, non-destructive state reconstruction using a single copy of the unknown state.
% 
    \textbf{(4) Hardware-aware implementation:} Unlike prior works that assume access to the density matrix of the unknown state or validate only on synthetic datasets, our method requires no such access and is compatible with noisy quantum hardware. This makes the approach both practical and scalable for NISQ devices.
% 
    \textbf{(5) Methods for State Deposition:} The primary objective of this work is to demonstrate multiple methods for performing state `deposition'. We present both gradient-based and gradient-free approaches: the former relies on gradient estimation to guide optimization, while the latter employs evolutionary strategies for state reconstruction. Depending on the context, the generated state may be represented as a state vector, a density matrix, or a unitary operator. 
% 
    \textbf{(6) Performance Evaluation:} \hl{add results}



% Given these limitations, a natural question arises: can quantum information be stored classically instead? 

% A pure quantum state can be fully specified (up to a global phase) by a normalized complex vector. 

% Although direct measurement collapses a quantum state, the SWAP test allows us to estimate the similarity between two quantum states without explicit knowledge of either. This opens an intriguing possibility: by iteratively generating candidate state vectors and comparing them to an unknown target using the SWAP test, one can reconstruct the original quantum state—up to a global phase, which is irrelevant for most quantum computing applications (refer to page 15 in \cite{Nielsen_Chuang_2010}).


% \subsection{Contribution}

% In this work, we explore this very idea. We present a machine learning-based framework that learns to reconstruct an unknown quantum state by generating state vectors and optimizing them based on their overlap with the target state. Once the correct state vector is found, it can be stored classically as a list of complex numbers. Later, this stored vector can be reloaded into a quantum circuit using standard state preparation techniques, such as the \texttt{StatePrep} method~\cite{StatePrep}, as implemented in PennyLane~\cite{bergholm_pennylane_2022} and related to the Möttönen transformation~\cite{mottonen_transformation_2004}.

% Through this approach, we demonstrate a method of classical storage and recovery of quantum information---not by freezing a quantum system in time, but by capturing and reconstructing its structure through data and learning. This work represents a step toward bridging the classical-quantum storage gap and opens new pathways in quantum information processing using hybrid approaches.

\subsection{Paper Structure}

The paper is organized as follows: Section II discusses related work. Section III details the proposed methods of quantum state deposition using gradient-based and gradient-free strategies. Section IV presents experimental results on both real hardware and simulations. Section V compares our method with existing approaches. Section VI outlines applications enabled by state withdrawal. Section VII discusses limitations and potential future directions. 


% So far we cannot store a quantum state classically because if a quantum state is measured it collapses into computational basis states and therefore it loses the quantum information. Current Qubits can not hold a state for long time due to short decoherence time. (citation needed). Therefore, Quantum memory technology is not realistically useful at the time of writing this paper. (add citations for these claims). However, having Quantum Memory elements will revolutionize the Quantum industry. There are many applications of Quantum Memory such as in Quantum Internet, Quantum communications, and Quantum repeaters, and so on. (add more examples with citations). 

% We can't store the Quantum information in Qubits currently for a long time but what if we can store the Quantum information classically? After all Quantum information is nothing but complex numbers.
% But we can not measure the Quantum State. But we can measure the overlap/similarity between two Quantum States using SWAP test. Now if we can generate State Vectors and check the similarity between the states until we find the right one then we will be able to find the unknown Quantum State and can represent that classically. 
% What if we can figure out what an unknown quantum state is, let's say in terms of the state vector, and then save the state vector which is nothing but complex number vectors, classically? Then when required we will load the state vector with a standard circuit synthesis method such as the Stateprep \cite{StatePrep} method in Pennylane \cite{bergholm_pennylane_2022}\cite{mottonen_transformation_2004}
% This is exactly what we achieved in this paper with the use of Machine Learning. We have developed an ML generator model that keeps generating the state vector until the correct state vector is generated. The correctness means the overlap between the states using the SWAP test and therefore it doesn't make sure the global phase is the same and which is not essential for two states to be effectively the same in quantum computing.  

==> junk.tex <==
% \subsection{Quantum Fidelity Estimation via Swap Test}

% To compute the fidelity between the unknown state and the generated candidate, we implement the swap test on a composite system of \( 2n + 1 \) qubits: an ancilla, a register for the unknown state, and a register for the generated state. The swap test is implemented as a \texttt{qml.qnode} circuit in \texttt{Pennylane}, using the following steps:

% \begin{enumerate}
%     \item Prepare the unknown and generated states on separate registers using \texttt{qml.StatePrep}.
%     \item Apply Hadamard and controlled-SWAP (CSWAP) gates controlled by the ancilla.
%     \item Measure the ancilla in the Pauli-Z basis. The expectation value provides an estimate of the fidelity through:
%     \[
%     F \approx 1 - 2P(0),
%     \]
%     where \( P(0) \) is the probability of measuring 0 on the ancilla.
% \end{enumerate}


% \subsection{Overview}
% Although gradient-based method reached fidelity ~1, it took a lot of manual tweaking of hyperparameters of the neural network and optimization. Specially for the noisy case, the gradients are very noise which makes training even harder and takes more epochs. Another reason for higher execution time is costly gradient calculations. Due to the fact SWAP test is non differentiable, we took resort to finite difference method which computes grdaients w.r.t every component of the state vector which is expensive in terms of number of execution of quantum circuits.  
% Therefore, we explored  gradient free method such as evolutionary strategies \cite{salimans_evolution_2017} and reinforcement learning. We couldn't make RL converge to higher fidelity and observed evolutionary strategies worked much better and was faster than gradient-based methods. 
% Therefore, we propose a variational approach for reconstructing an unknown quantum state vector by maximizing its fidelity with a learned approximation, using an Evolutionary Strategy (ES) algorithm guided by swap-test fidelity. Our method is implemented using \texttt{Pennylane} and \texttt{PyTorch}, leveraging both classical and quantum components to iteratively optimize the State Vector/ density matrix representation of the quantum state.
% Although gradient-based methods achieved fidelities close to 1 in noiseless simulations, this required extensive manual tuning of the neural network's hyperparameters and the optimization procedure. This challenge was particularly pronounced in the presence of noise, where gradients became unstable, making training more difficult and requiring a larger number of epochs to converge and for higher qubits the fidelity went close to 0.85 not 0.99. 

% Another contributing factor to the high execution time was the cost of gradient computation. Since the SWAP test is non-differentiable, we resorted to finite difference methods to estimate gradients with respect to each component of the state vector. This approach is computationally expensive, as it demands a large number of quantum circuit executions.




% \section*{References}

% Please number citations consecutively within brackets \cite{b1}. The 
% sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
% number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
% the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

% Number footnotes separately in superscripts. Place the actual footnote at 
% the bottom of the column in which it was cited. Do not put footnotes in the 
% abstract or reference list. Use letters for table footnotes.

% Unless there are six authors or more give all authors' names; do not use 
% ``et al.''. Papers that have not been published, even if they have been 
% submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
% that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
% Capitalize only the first word in a paper title, except for proper nouns and 
% element symbols.

% For papers published in translation journals, please give the English 
% citation first, followed by the original foreign-language citation \cite{b6}.

% \begin{thebibliography}{00}
% \bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
% \bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
% \bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
% \bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
% \bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
% \bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
% \bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
% \bibitem{b8} D. P. Kingma and M. Welling, ``Auto-encoding variational Bayes,'' 2013, arXiv:1312.6114. [Online]. Available: https://arxiv.org/abs/1312.6114
% \bibitem{b9} S. Liu, ``Wi-Fi Energy Detection Testbed (12MTC),'' 2023, gitHub repository. [Online]. Available: https://github.com/liustone99/Wi-Fi-Energy-Detection-Testbed-12MTC
% \bibitem{b10} ``Treatment episode data set: discharges (TEDS-D): concatenated, 2006 to 2009.'' U.S. Department of Health and Human Services, Substance Abuse and Mental Health Services Administration, Office of Applied Studies, August, 2013, DOI:10.3886/ICPSR30122.v2
% \bibitem{b11} K. Eves and J. Valasek, ``Adaptive control for singularly perturbed systems examples,'' Code Ocean, Aug. 2023. [Online]. Available: https://codeocean.com/capsule/4989235/tree
% \end{thebibliography}

==> memory_bank_tex/application_memory_bank.tex <==
\subsection{Quantum State Tomography}
Measurement comparison with QST technology

\subsubsection{Background: What is Quantum State Tomography (QST)?}

Quantum State Tomography (QST) is the process of reconstructing a quantum state $\rho$ from a complete set of measurement outcomes. For a pure state $\ket{\psi} \in \mathbb{C}^{2^n}$, QST involves performing measurements in multiple bases, collecting statistics over repeated experiments, and solving an inverse problem (e.g., via maximum likelihood estimation or convex optimization) to recover the state.

\vspace{1ex}
\noindent
However, QST suffers from several major bottlenecks:
\vspace{-0.5ex}
\begin{itemize}
  \setlength\itemsep{0.2em}
  \item \textbf{Exponential scaling:} The number of required measurements grows exponentially with the number of qubits: at least $\mathcal{O}(4^n)$ parameters are needed to describe a general mixed state.
  \item \textbf{Measurement overhead:} A full set of tomographic measurements must be performed in all combinations of Pauli bases.
  \item \textbf{Post-processing complexity:} Reconstructing the density matrix or pure state involves solving a high-dimensional inverse problem.
  \item \textbf{Noise sensitivity:} Measurement errors and statistical fluctuations can significantly degrade reconstruction fidelity.
\end{itemize}

\vspace{1ex}
\noindent
\textbf{Advantages of Our Method:} Our proposed method replaces the measurement-heavy QST pipeline with a learning-based approach, which optimizes a neural model to generate the unknown state by directly maximizing fidelity via quantum circuits (e.g., the swap test). Below are detailed comparisons across key dimensions in Table \ref{table1}

% \begin{table*}[h!]\label{table1}
% \centering
% \caption{Comparison between Traditional Quantum State Tomography and Our Fidelity-Based Learning Method}
% \begin{tabular}{|p{2cm}|p{7cm}|p{7cm}|}
% \hline
% \textbf{Feature} & \textbf{Traditional Quantum State Tomography} & \textbf{Our Fidelity-Based Learning Method} \\
% \hline
% \textbf{Measurement Complexity} & Requires $O(3^n)$ measurement settings across multiple bases (X, Y, Z) & Requires only one observable (Pauli-Z on control qubit in swap test) \\
% \hline
% \textbf{Scalability with Qubits} & Poor scalability due to exponential growth in measurements and reconstruction complexity & Good scalability; uses $2n+1$ qubits in swap test and avoids exponential post-processing \\
% \hline
% \textbf{Noise Robustness} & Sensitive to SPAM errors and statistical noise; requires regularization & Robust to noise via iterative optimization and fidelity smoothing \\
% \hline
% \textbf{Training Feedback} & Passive; all data collected before reconstruction & Active; model receives fidelity-based feedback each iteration \\
% \hline
% \textbf{Computational Overhead} & High classical cost for density matrix estimation or MLE & Minimal; no post-processing, output is directly learned \\
% \hline
% \textbf{Generalization Capability} & None; each state treated independently & Can generalize across families of states if trained appropriately \\
% \hline
% \textbf{Data Reusability} & No reuse of measurements once collected & Training inherently reuses data via backpropagation \\
% \hline
% \textbf{Best Use Case} & Full tomography of low-qubit mixed states & Pure or low-rank states where fidelity is sufficient \\
% \hline
% \end{tabular}
% \end{table*}

% \subsection{Mid Circuit Measurement, Snapshot}


\subsection{Application to Mid-Circuit Measurement and Quantum Snapshots}

As quantum hardware evolves, mid-circuit measurements (MCM) and quantum snapshots are becoming essential tools for enabling feedback-based computation, error detection, adaptive protocols, and time-evolving state tracking. These operations allow partial access to the state of a quantum system during the course of a computation, without collapsing the entire wavefunction.

Our proposed method---reconstructing quantum states using a neural generator trained via the swap test---offers unique benefits in both these contexts.

\subsubsection{Quantum Snapshot Reconstruction}

A quantum snapshot refers to a partial or complete capture of the state of a quantum system at an intermediate point in a quantum circuit. This is often used for:
\begin{itemize}
    \item Debugging and circuit introspection
    \item Tracking state evolution in time-dependent processes
    \item Verifying the correctness of variational protocols
\end{itemize}

However, in practical devices, taking full snapshots (via tomography) is infeasible due to resource costs.

\paragraph{How Our Method Helps} Given access to the quantum state at an intermediate point in the circuit (e.g., via a saved vector or partial tomography), we can train a generator model to replicate that snapshot.

Using our swap-test-based fidelity loss, the generator can be optimized to recreate the snapshot state without requiring repeated destructive measurements.

Once trained, this generator acts as a compact, reusable representation of the intermediate quantum state, useful for debugging, state injection, or later analysis.

This avoids the cost of storing large state vectors and instead provides a learned, parameter-efficient encoding of the state at that point in the circuit.

\subsubsection{Mid-Circuit Measurement and Adaptive State Tracking}

Mid-circuit measurements allow specific qubits to be measured during computation and then reused or modified conditionally, enabling:
\begin{itemize}
    \item Error mitigation and detection
    \item Adaptive measurement strategies
    \item Measurement-based quantum computation
\end{itemize}

However, these measurements can disrupt the remaining quantum state, and their outcomes are often stochastic. In such settings, learning to predict or approximate the post-measurement state becomes important.

\paragraph{How Our Method Helps} Suppose a mid-circuit measurement is made on a subset of qubits, collapsing the state to a known branch conditioned on the measurement result.

The remaining unmeasured qubits are in a projected (but unknown) state.

Our method can reconstruct this projected post-measurement state by treating it as the new unknown 
\(|\psi\rangle\), and learning a generator that replicates it with high fidelity.

This is particularly useful in:
\begin{itemize}
    \item Quantum simulations, where adaptive branching occurs
    \item Error decoding, where one wants to learn the most probable state after syndrome measurement
    \item Quantum control, where the system evolves depending on feedback and state collapse
\end{itemize}

Moreover, since mid-circuit measurement often involves conditional operations, we can treat the measurement outcome as a condition \(z\), and train a conditional generator \(G(z)\) that learns to generate the correct projected state based on classical measurement history.







\subsection{Circuit Optimization}
\subsection{Quantum Repeater}
\subsection{Quantum Sensor}

==> memory_bank_tex/results_memory_bank.tex <==
We have tested our hypothesis in real hardware (IBM Superconducting qubits), noisy simulations using IBM hardware noise models, and noiseless simulations using AerSimulator in Pennylane. 

% Due to lack of resources in real hardware we have verified few 1 qubit known states such as states |0> = [1, 0], |1> = [0, 1], Bell State = 1/ \sqrt{2}[1,1] and we achieved fidelity of 1 within 3 epochs. 
Due to lack of resources on real hardware, we have verified a few known single-qubit states, such as the states $\ket{0} = [1, 0]$, $\ket{1} = [0, 1]$, and the Hadamard state $\frac{1}{\sqrt{2}}[1, 1]$. We achieved a fidelity of $1$ within $3$ epochs.

We have executed extensive experiments using both noisy and noiseless simulation which results are presented below. 
\input{results_noisemodel_memory_bank}

\subsection{Noisy and Noiseless Simulation Experiments}
\subsubsection{Distribution between Target and Reconstructed State Fidelity}
\ref{fig:statevector_unitary_fidelity_distribution} shows fidelity values as per \ref{fidelity}. The fidelity was calculated by randomly sampling 1000 states, and then the corresponding fidelity was reported from the noiseless simulation using the Qiskit AerSimulator. The results show that the min fidelity achieved is 99.9\% which is much better than the SOTA method 99.1 \% \cite{liu_variational_2020} and it is achieved much faster within 30 epochs. (some of them reached to best fidelity much earlier and we did early stopping for those cases.  ) 
\hl{TBD: Plot qubit vs epoch needed and time needed}
% \begin{figure}[]
%     \centering
%     \includegraphics[width=1\linewidth]{fig/statevector_unitary_fidelity_distribution.pdf}
%     \caption{Statevector unitary fidelity distribution}
%     \label{fig:statevector_unitary_fidelity_distribution}
% \end{figure}

% Here is a comparison table across various literature and our work.

% \begin{table}[h]
% \centering
% \begin{tabular}{|l|c|c|c|}
% \hline
% \textbf{Metric} & \textbf{Our Approach} & \textbf{Liu et al.} & \textbf{Paper 3} \\
% \hline
% Min Fidelity Achieved & 99.9\% & 99.1\% & -- \\
% \hline
% Epochs & 30 (max) & -- & -- \\
% \hline
% Number of Shots & -- & -- & -- \\
% \hline
% Noisy Sim Fidelity & -- & X & X \\
% \hline
% Noisy Sim Epochs & -- & X & X \\
% \hline
% Noisy Sim Shots & -- & X & X \\
% \hline
% Hardware Results & Yes & No & No \\
% \hline
% \end{tabular}
% \caption{Comparison of Quantum State Reconstruction Results Across Papers}
% \label{tab:paper_comparison}
% \end{table}


Find the 6-sigma value and other stat values
\subsubsection{Amplitude Comparison of Target and Reconstructed States }
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/amplitude_3d_plot.pdf}
    \caption{Amplitude Comparison of Target and Reconstructed States}
    \label{fig:amplitude_3d_plot}
\end{figure}
We have picked a couple of states to show that amplitude probabilities in 2 qubit basis states are almost same which reiterates the fact fidelity is high and also the right measure to compare similarity between quantum states. 
\subsubsection{Entanglement Quality of Target and Reconstructed States }
In order to determine whether our unknown target states are sufficiently entangled, we measured the entanglement entropy of those states using the following method. We calculated the von Neumann entropy of the reduced density matrix obtained by performing a bipartition of the system. Specifically, for a given pure state $\lvert\psi\rangle$, we traced out half of the system to obtain the reduced density matrix $\rho_A = \mathrm{Tr}_B(\lvert\psi\rangle\langle\psi\rvert)$, and then computed the entanglement entropy as
\[
S(\rho_A) = -\mathrm{Tr}(\rho_A \log \rho_A).
\]
This entropy quantifies how entangled a state is across the chosen bipartition.

We observed a good mixture of highly entangled states and matrix product states with low entanglement. Notably, the reconstructed states exhibited entanglement properties closely matching those of the corresponding unknown target states. This confirms the robustness of our method across a range of entangled and weakly entangled (matrix product) states. Figure~4 (left) displays the entanglement entropy of the target states, while Figure~4 (right) demonstrates that the entanglement entropy of the generated states aligns well with that of the target states. This strong agreement further supports that the generated states faithfully capture the entanglement structure of the target states.

\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{fig/statevector_entanglement_entropy.pdf}
    \caption{Statevector entanglement entropy}
    \label{fig:statevector_entanglement_entropy}
\end{figure}

\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{fig/statevector_fidelity_distribution.pdf}
    \caption{Statevector fidelity distribution}
    \label{fig:statevector_fidelity_distribution}
\end{figure}

\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{fig/unitary_fidelity_distribution.pdf}
    \caption{Unitary fidelity distribution}
    \label{fig:unitary_fidelity_distribution}
\end{figure}

\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{fig/density_matrix_fidelity_distribution.pdf}
    \caption{Density matrix with fidelity and ulhman fidelity}
    \label{fig:density_matrix_fidelity_distribution}
\end{figure}

\subsubsection{Calculation of total number of shots/copy}
\subsubsection{Transferability of Model}
We explored the pretraining of models by initially training a single model on 1000 randomly generated quantum states. This pre-trained model was then evaluated on a separate set of 100 unknown and known quantum states, as summarized in Table~\ref{tab:quantum_state_result}. We observed an average improvement of approximately $70\%$ in the number of epochs required to reach a comparable fidelity.

\subsection{Comparison}

\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{fig/grouped_barplot_correct_order.pdf}
    \caption{State Vector}
    \label{fig:grouped_barplot_correct_order}
\end{figure}

\input{table_master_results}
\input{table_big_state}























==> memory_bank_tex/results_noisemodel_memory_bank.tex <==
\subsection{Noisemodel}
% \subsection*{Noise Model Specification}

% To emulate the behavior of near-term quantum devices, we incorporate a customized noise model based on Qiskit's \texttt{NoiseModel} framework. This model captures both gate-dependent and qubit-specific imperfections, enabling the simulation of quantum circuits under realistic conditions. The key properties of the noise model are as follows:

% \begin{itemize}
%     \item \textbf{Supported Gate Set}: The noise model operates over the following basis gates:
%     \[
%     \{\texttt{cx},\ \texttt{delay},\ \texttt{id},\ \texttt{measure},\ \texttt{reset},\ \texttt{rz},\ \texttt{sx},\ \texttt{x}\}
%     \]
%     These include both native quantum operations and auxiliary operations such as idle and measurement.

%     \item \textbf{Noisy Operations}: Noise is explicitly modeled for a subset of these gates:
%     \[
%     \{\texttt{id},\ \texttt{cx},\ \texttt{x},\ \texttt{measure},\ \texttt{sx}\}
%     \]
%     This implies that these operations incur gate-specific decoherence or stochastic errors.

%     \item \textbf{Noisy Qubits}: The model includes noise on all physical qubits. Each qubit is subject to noise depending on the operation applied.

%     \item \textbf{Instruction-Specific Noise Mapping}: The noise model specifies fine-grained gate-qubit combinations. For instance:
%     \begin{itemize}
%         \item Two-qubit errors are defined for \texttt{cx} gates between all pairwise combinations, such as \texttt{cx}(0,1), \texttt{cx}(2,3), etc., to simulate entangling gate infidelities.
%         \item Single-qubit noise affects identity operations (\texttt{id}) to model \textit{idle decoherence}, as well as gates like \texttt{x}, \texttt{sx}, and \texttt{measure} to simulate \textit{unitary errors} and \textit{readout noise}.
%     \end{itemize}
% \end{itemize}



% \subsection*{Impact on Quantum State Reconstruction}

% In our setting, this noise model plays a crucial role in evaluating the quality of reconstructed quantum states. Specifically, it impacts:
% \begin{itemize}
%     \item \textbf{State preparation circuits}, used by the generative model to produce candidate quantum states;
%     \item \textbf{Fidelity estimation via the swap test}, which acts as the primary loss function;
%     \item \textbf{Gradient-based training routines}, where parameter updates must remain robust to statistical fluctuations introduced by noise.
% \end{itemize}

% By incorporating this detailed noise structure, our learning framework becomes both device-aware and resilient to hardware-induced infidelities, facilitating accurate and transferable quantum state reconstruction in the NISQ regime.

% 


To realistically simulate the behavior of near-term noisy quantum processors, we incorporate a detailed gate-level noise model derived from an IBM GenericBackendV2 for the required number of qubits. This model is integrated using Qiskit's \texttt{NoiseModel} interface and imported into PennyLane via a custom Aer device. The key features of the model are outlined below:

\begin{itemize}
    \item \textbf{Basis Gate Set}: The noise model supports the following native operations:
    \[
    \{\texttt{cx},\ \texttt{delay},\ \texttt{id},\ \texttt{measure},\ \texttt{reset},\ \texttt{rz},\ \texttt{sx},\ \texttt{x}\}
    \]
    
    \item \textbf{Noisy Instructions}: Noise is defined on a subset of these operations:
    \[
    \{\texttt{id},\ \texttt{cx},\ \texttt{sx},\ \texttt{x},\ \texttt{measure}\}
    \]
    indicating that idle operations, single-qubit unitaries, and two-qubit entangling gates are all subject to non-trivial noise processes.

    \item \textbf{Qubits with Noise}: All qubits indexed as \( q_0, q_1, q_2, q_3 ... q_n \) are affected by gate-dependent noise.

    \item \textbf{Gate-Qubit Error Map}: The noise model provides fine-grained control over qubit-specific gate errors via \texttt{QubitChannel} representations. These channels internally encode Kraus operators to simulate stochastic quantum noise. For instance:
    \begin{itemize}
        \item CNOT gates between qubit pairs exhibit asymmetric noise profiles. For example:
        \begin{itemize}
            \item \texttt{cx}(0,1): \texttt{QubitChannel} with 16 Kraus operators
            \item \texttt{cx}(0,2): \texttt{QubitChannel} with 9 Kraus operators
        \end{itemize}
        \item Single-qubit gates such as \texttt{id}, \texttt{sx}, and \texttt{x} apply noisy channels using 3 to 4 Kraus operators.
    \end{itemize}

    \item \textbf{Asymmetric Noise Modeling}: The number of Kraus operators varies across different gates and qubit pairs, reflecting real device asymmetries in gate infidelity. This captures not only gate-dependent but also hardware-layout-specific noise behavior.
    
    % \item \textbf{Readout Noise Warning}: While the noise model includes readout noise channels for \texttt{measure} operations, current limitations in PennyLane's Qiskit interface result in these channels being skipped during simulation:
    % \begin{quote}
    % \texttt{UserWarning: Readout errors are not supported currently and will be skipped.}
    % \end{quote}
    % Therefore, measurement errors are not simulated explicitly.
\end{itemize}

This nuanced noise model enables us to perform variational training and quantum state reconstruction under physically realistic conditions. By introducing non-uniformity in fidelity degradation across gates and qubit pairs, the model better represents the noise anisotropy observed in superconducting qubit architectures. It thus provides a critical tool for benchmarking algorithmic robustness, especially when optimizing under the fidelity loss metric derived from the swap test.

In Table~\ref{tab:noisemodel}, we provide a summary of the noise model corresponding to a 5-qubit quantum circuit, adapted from an IBM 5-qubit quantum backend. This configuration reflects a dense interaction topology and non-trivial noise distribution, characteristic of real IBMQ processors such as \texttt{ibmq\_quito} or \texttt{ibmq\_lima}. It enables us to assess the performance of quantum algorithms under realistic, gate-dependent, and correlated noise conditions.

\begin{table*}[h!]
\centering
\caption{5 Qubit Qiskit Noise Model Summary}
\begin{tabular}{c|c|c}

\textbf{Gate Type} & \textbf{Qubits Affected} & \textbf{Noise Description} \\
\hline \hline
\texttt{id}       & $q_0, q_1, q_2, q_3, q_4$ & Idle decoherence \\ \hline
\texttt{x}        & $q_0, q_1, q_2, q_3, q_4$ & Bit-flip or unitary gate noise \\ \hline
\texttt{sx}       & $q_0, q_1, q_2, q_3, q_4$ & Under/over-rotation errors \\ \hline
\texttt{measure}  & $q_0, q_1, q_2, q_3, q_4$ & Readout error (bit-flip) \\ \hline
\texttt{cx}       & All pairs of 2-qubit combinations among $q_0$–$q_4$ & Entangling gate noise \\
\hline \hline
\end{tabular}
\label{tab:noisemodel}
\end{table*}

==> methods_memory_bank.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{fig/bloch_sphere.pdf}
    \caption{Progression of reconstructed states towards target states for noiseless and noisy condition}
    \label{fig:bloch_sphere}
\end{figure}
% First, we show explain our methods to find out an unknown state at any dissection of the quantum circuit and after that we save that state classically in a classical memory. 
% We propose three methods for quantum state regeneration, each accompanied by two distinct estimation techniques: a gradient-based approach using a deep learning generator, and a gradient-free approach leveraging evolutionary strategies.
% First, we describe our methods for identifying an unknown quantum state at any intermediate point within a quantum circuit. Once the state is estimated, it is stored classically in a conventional memory for future use.

% To enable state estimation, we propose three distinct methods to represent and reconstruct states, each supported by two estimation strategies: a gradient-based technique utilizing a deep learning generator, and a gradient-free approach based on evolutionary strategies.

% We generate states by State Vector, Density matrix, and Unitary matrix which can transform a state $\ket{0} $ to state $\ket{\psi} $. We use our estimation methods to estimate these three types of representation of a state. 

% Here first we explain using gradient based method to estimate a State vector and the with gradient free method, Evolutionary Strategies. The same method goes for both density matrix generation and Unitary generation. Only difference is the density and unitary matrix are 2^n *2 ^n matrix whereas state vectors are $\ket{\psi} \in \mathbb{C}^{2^n}$ 
We begin by presenting our framework for identifying an unknown quantum state at any intermediate stage of a quantum circuit. Once estimated, the state is stored classically in conventional memory, enabling its later reconstruction when needed.

To facilitate state estimation, we tried three distinct methods for representing and regenerating quantum states:
\begin{enumerate}
    \item \textbf{State vector representation}, for Pure State  
    \item \textbf{Density matrix representation}, for Pure state and mixed state and
    \item \textbf{Unitary matrix representation}—where the unitary transforms the initial state $\ket{0}^{\otimes n}$ to the target state $\ket{\psi}$.
\end{enumerate}

Each of these representations is reconstructed using two estimation strategies:
\begin{itemize}
    \item A \textbf{gradient-based method} employing a deep learning generator trained via backpropagation, and
    \item A \textbf{gradient-free method} utilizing evolutionary strategies for optimization.
\end{itemize}

In the case of the \textit{state vector}, we directly estimate $\ket{\psi} \in \mathbb{C}^{2^n}$. For the \textit{density matrix} and \textit{unitary matrix}, we estimate complex-valued matrices of size $2^n \times 2^n$, subject to appropriate constraints (e.g., Hermiticity and trace-one for density matrices, unitarity for unitaries).

We first detail the gradient-based approach for estimating the state vector, followed by its gradient-free counterpart. The same estimation framework is then extended to density matrix and unitary generation, with adaptations to accommodate the higher-dimensional structure and relevant physical constraints of each representation.

We describe the procedure for generating the state vector in detail. This approach naturally extends to the other two cases: unitary and density matrix representations. While we provide the overall process in pseudocode, detailed explanations are omitted due to space constraints.
%\subsection{The three methods to represent and reconstruct states }

\begin{algorithm}[H]
\caption{Statevector based Fidelity Estimation}
\begin{algorithmic}[1]
\Require Number of qubits $N$, epochs $E$
\State $d \gets 2^N$
\State Initialize neural network $\mathcal{F}_\theta: \mathbb{R} \to \mathbb{C}^d$
\State Sample target state $\ket{\psi} \in \mathbb{C}^d$ and normalize

\For{epoch $= 1$ to $E$}
    \State $z \gets \mathcal{U}(0, 1)^{256}$
    \State $\ket{\phi_\theta} \gets \mathcal{F}_\theta(z)$
    \State Use SWAP test to estimate fidelity $F = |\bra{\psi}\ket{\phi_\theta}|^2$
    \State Compute loss: $\mathcal{L} = 1 - F$
    \State Update $\theta$ using gradient descent
    \If{$F = \sim 1.0$}
        \State \textbf{break}
    \EndIf
\EndFor

\State \Return final fidelity $F$
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[H]
\caption{Unitary based Fidelity Estimation}
\begin{algorithmic}[1]
\Require Number of qubits $N$, epochs $E$
\State $d \gets 2^N$, $p \gets 2d^2$
\State Initialize neural network $\mathcal{G}_\theta: \mathbb{R} \to \mathbb{R}^p$
\State Sample target unitary $U_{\text{target}} \in \mathbb{C}^{d \times d}$

\For{epoch $= 1$ to $E$}
    \State Sample random noise $z$
    \State $\vec{v} \gets \mathcal{G}_\theta(z)$
    \State Construct complex matrix $M$ from $\vec{v}$
    \State $U_\theta \gets \text{QR-decomposition}(M)$
    \State Use SWAP test to estimate fidelity $F = |\bra{U_{\text{target}}} \ket{U_\theta}|^2$
    \State Compute loss: $\mathcal{L} = 1 - F$
    \State Update $\theta$ using gradient descent
    \If{$F =\sim 1.0$}
        \State \textbf{break} 
    \EndIf
\EndFor

\State \Return final fidelity $F$
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[H]
\caption{Density Matrix-based Fidelity Estimation}
\begin{algorithmic}[1]
\Require Number of qubits $Q$, epochs $E$
\State $d_1 \gets 2^Q$, $d_2 \gets 2^{2Q}$, $p \gets 2d_2^2$
\State Initialize neural network $\mathcal{G}_\theta: \mathbb{R} \to \mathbb{R}^p$
\State Sample target mixed state \( \rho_{\text{target}} \in \mathbb{C}^{d_1 \times d_1} \)

\For{epoch $= 1$ to $E$}
    \State Sample random noise $z$
    \State $\vec{v} \gets \mathcal{G}_\theta(z)$
    \State Construct complex matrix $M$ from $\vec{v}$
    \State $\rho_\theta \gets Construct\_Mixed\_State(M)$
    \State Use SWAP test to estimate fidelity $F = |\langle \rho_{\text{target}} | \rho_\theta \rangle|^2$
    \State Compute loss: $\mathcal{L} = 1 - F$
    \State Update $\theta$ using gradient descent
    \If{$F = \sim 1.0$}
        \State \textbf{break}
    \EndIf
\EndFor

\State \Return final fidelity $F$
\end{algorithmic}
\end{algorithm}
\subsection{Gradient Based Method: Deep Learning Model as Generator}

\subsubsection{Problem Formulation}
%or density matrix $\ket{\psi} \in \mathbb{C}^{2^n \times 2^n}$ or unitary matrix $2^n \times 2^n$
The goal of this work is to reconstruct an unknown quantum state vector 
$\ket{\psi} \in \mathbb{C}^{2^n}$  given no prior information about its structure, by leveraging a machine learning (ML) model. Specifically, we aim to train a model that can generate a quantum state $\ket{\phi}$ such that the fidelity 
\begin{equation}
F = |\bra{\psi}\ket{\phi}|^2
\end{equation}
approaches unity. This indicates that the generated state is indistinguishable from the unknown state (global phase difference doesn't matter).

We develop a deep neural network model where the generator generates the states intending to match with unknown target state and the SWAP test acts like a loss function telling how far the generated state is similar to the target unknown state thus guiding the generator to train towards generating correct state which brings fidelity between quantum states 1. 

% \subsection{Overview of the Method}
% Our proposed pipeline includes the following components:
% \begin{itemize}
%     \item Generation of a normalized, randomly sampled unknown quantum state $\ket{\psi}$ and corresponding quantum circuit as a proxy of real life unknown quantum State,
%     \item A neural network-based generator that outputs candidate quantum states $\ket{\phi}$,
%     \item A quantum swap test circuit for evaluating the fidelity between $\ket{\psi}$ and $\ket{\phi}$,
%     \item A loss function based on fidelity maximization,
%     \item Gradient-based optimization of the model using backpropagation through a classical generator ML model.
% \end{itemize}
\subsubsection{Overview of the Method}

Our proposed pipeline enables the dynamic reconstruction of an unknown quantum state using mid-circuit fidelity estimation. The key components of the method are as follows:

\begin{enumerate}
    \item \textbf{Unknown state preparation:} A normalized, randomly sampled quantum state $\ket{\psi}$ is generated along with its corresponding quantum circuit. This serves as a proxy for an unknown quantum state encountered in real computation.
    
    \item \textbf{Classical neural network generator:} A classical neural network is trained to output a candidate state vector $\ket{\phi}$. The output is normalized and used to construct a quantum circuit using the Mottonen state preparation method~\cite{mottonen_transformation_2004}, implemented via \texttt{qml.StatePrep}~\cite{noauthor_qmlstateprep_nodate}.
    
    \item \textbf{Fidelity estimation via SWAP test:} The overlap between $\ket{\psi}$ and $\ket{\phi}$ is evaluated using a quantum SWAP test. This test is implemented with mid-circuit measurements, enabling real-time fidelity estimation without disturbing the target state until necessary.
    
    \item \textbf{Loss function and training:} The fidelity estimated from the SWAP test is used to define a loss function that encourages the neural network to produce states with maximal overlap with the unknown target. The model is trained using gradient-based optimization and finite-difference gradient estimation due to the non-differentiable quantum components.
    
    \item \textbf{Classical storage and retrieval:} Once a candidate state $\ket{\phi}$ achieves high fidelity with the unknown state $\ket{\psi}$, it is saved as a classical vector. This representation can later be reloaded and re-prepared on quantum hardware using standard QRAM-compatible algorithms, laying the foundation for classically stored quantum memory.
\end{enumerate}

\subsubsection{Unknown Quantum State Generation}
We simulate an arbitrary, unknown quantum state $\ket{\psi}$ over $n$ qubits. The state vector is randomly sampled from the complex unit sphere in $\mathbb{C}^{2^n}$. The real and imaginary components of each amplitude are independently sampled from a standard normal distribution. The state vector is then normalized to unit length:
\begin{equation}
\ket{\psi} = \frac{\vec{r} + i \vec{i}}{\|\vec{r} + i \vec{i}\|}
\end{equation}
where $\vec{r}, \vec{i} \in \mathbb{R}^{2^n}$ are drawn from $\mathcal{N}(0,1)$.

% \subsection{Quantum State Generator Model}
% To generate candidate quantum states, we implement a feedforward neural network parameterized by weights $\theta$. The model maps a latent input vector $z \in \mathbb{R}$ to a complex-valued output vector in $\mathbb{C}^{2^n}$, representing the amplitudes of a quantum state.

% The model includes:
% \begin{itemize}
%     \item Two linear layers with ReLU activation,
%     \item A final layer outputting $2 \cdot 2^n$ values (real and imaginary components),
%     \item Normalization of the output within the quantum circuit using PennyLane's \texttt{StatePrep}.
% \end{itemize}

% Formally, the generator is defined as:
% \begin{equation}
% \phi_{\theta}(z) = \text{Normalize}\left( \text{ReLU}\left( W_2 \left( \text{ReLU}(W_1 z + b_1) \right) + b_2 \right) \right)
% \end{equation}
% where $\phi_{\theta}(z)$ is interpreted as the generated quantum state vector.
\subsubsection{Generator Architecture}

The quantum state generator is implemented as a deep fully connected neural network, \texttt{QuantumStateGenerator}, using PyTorch. It takes as input a 256-dimensional latent vector \( \mathbf{z} \) and outputs a real-valued vector of dimension \( 2 \times \texttt{dim} \), where \texttt{dim} denotes the number of complex amplitudes in the target quantum state. The output vector is interpreted as the concatenation of the real and imaginary components of the generated quantum state.

The architecture comprises six linear layers interleaved with GELU (Gaussian Error Linear Unit) activations, except at the output. The layer-wise progression is as follows:
\begin{align*}
\text{Linear}(256 \rightarrow 512) &\rightarrow \text{GELU} \\
\text{Linear}(512 \rightarrow 1024) &\rightarrow \text{GELU} \\
\text{Linear}(1024 \rightarrow 1024) &\rightarrow \text{GELU} \\
\text{Linear}(1024 \rightarrow 512) &\rightarrow \text{GELU} \\
\text{Linear}(512 \rightarrow 256) &\rightarrow \text{GELU} \\
\text{Linear}(256 \rightarrow 2 \times \texttt{dim}) &
\end{align*}

\subsubsection{Fidelity-Based Optimization via Swap Test}\label{swap_test}

To evaluate the similarity between the generated quantum state and the unknown target state, we employ a fidelity measure based on the quantum \textit{swap test}. Given two quantum states \( \lvert \psi \rangle \) and \( \lvert \phi \rangle \), the swap test estimates the fidelity as:
\[
F(\psi, \phi) = |\langle \psi | \phi \rangle|^2,
\]
which serves as the primary optimization objective during training.

The swap test uses $2n + 1$ qubits:
\begin{itemize}
    \item Qubits $1$ to $n$: initialized with $\ket{\psi}$,
    \item Qubits $n+1$ to $2n$: initialized with $\ket{\phi}$,
    \item Qubit $0$: control qubit used for controlled-swap operations.
\end{itemize}

The expected value of the Pauli-Z observable on the control qubit gives:
\begin{equation}\label{fidelity}
% \langle Z \rangle = 2|\bra{\psi}\ket{\phi}|^2 - 1 \quad \Rightarrow \quad F = \frac{1 + \langle Z \rangle}{2}
\langle Z \rangle = |\bra{\psi}\ket{\phi}|^2 \quad \Rightarrow \quad F = \langle Z \rangle
\end{equation}

Since the standard swap test is non-differentiable, we implement a custom autograd function, \texttt{SwapTestFunction}, which uses finite-difference approximation to compute gradients. In the forward pass, the real and imaginary components of the generated output are combined to form a complex-valued state vector, which is normalized to unit norm. The fidelity is then computed between this state and the unknown target.

During the backward pass, each element of the generated output is perturbed slightly in both directions to estimate the gradient via symmetric finite differences. This approach allows us to propagate gradients through the fidelity computation and train the network using standard gradient-based optimization methods.

\subsubsection{Combined Model}

The complete model, \texttt{QuantumStateLearningModel}, integrates the generator and fidelity evaluation into a unified architecture. It receives a latent vector \( \mathbf{z} \) and an unknown target state as input and returns both the fidelity score and the normalized generated quantum state. The model is trained to maximize the fidelity, while the generated state is preserved for downstream use in quantum circuit construction.

\subsubsection{Training Procedure}

We train the model using the Adam optimizer with a learning rate of \( 1 \times 10^{-4} \). The loss function is defined as:
\[
\mathcal{L} = 1 - F,
\]
where \( F \) is the fidelity between the generated and target states.

At each training step, a latent vector \( \mathbf{z} \sim \mathcal{U}(0, 1)^{256} \) is sampled from a uniform distribution. The generator maps this vector to a complex-valued quantum state, and the fidelity with the target state is evaluated. The computed loss is then backpropagated through the custom autograd function.

To stabilize training, all gradients are manually scaled by a constant \texttt{scaling\_factor} before each optimizer step. The training loop is executed for a fixed number of epochs (depending on the number of qubits), and the best fidelity observed across all epochs is recorded as a key performance indicator.

% \subsection{Fidelity Estimation via Swap Test}
% To evaluate the similarity between the generated and the unknown states, we use the swap test—an algorithm for estimating inner products between quantum states. The swap test uses $2n + 1$ qubits:
% \begin{itemize}
%     \item Qubits $1$ to $n$: initialized with $\ket{\psi}$,
%     \item Qubits $n+1$ to $2n$: initialized with $\ket{\phi}$,
%     \item Qubit $0$: control qubit used for controlled-swap operations.
% \end{itemize}

% The expected value of the Pauli-Z observable on the control qubit gives:
% \begin{equation}\label{fidelity}
% % \langle Z \rangle = 2|\bra{\psi}\ket{\phi}|^2 - 1 \quad \Rightarrow \quad F = \frac{1 + \langle Z \rangle}{2}
% \langle Z \rangle = |\bra{\psi}\ket{\phi}|^2 \quad \Rightarrow \quad F = \langle Z \rangle
% \end{equation}

% This circuit is implemented using the PennyLane framework with automatic differentiation for end-to-end optimization.

% \subsection{Loss Function and Optimization}
% The loss function is defined as:
% \begin{equation}
% \mathcal{L} = 1 - F = 1 - |\bra{\psi}\ket{\phi}|^2
% \end{equation}

% Minimizing this loss maximizes the fidelity between the generated and target state vectors. We train the model using the Adam optimizer with a learning rate of $0.001$. For simplicity, a single latent input vector $z = [1.0]$ is used, though the approach generalizes to higher-dimensional latent spaces.

% \subsection{Training Procedure}
% The training loop runs for 150 epochs. In each iteration:
% \begin{itemize}
%     \item A candidate quantum state is generated by the model,
%     \item The swap test circuit estimates fidelity,
%     \item The loss is computed and backpropagated,
%     \item The model parameters are updated using Adam.
% \end{itemize}

% Fidelity is logged at each step. We stop the training when fidelity reaches a certain user-defined threshold (ex: 0.99999999) or the number of predetermined epochs are over. 

\subsubsection{Final Evaluation}
After training, The final state is compared classically to the target state via the inner product $|\bra{\psi}\ket{\phi}|^2$ for validation.

A fidelity value close to $1$ indicates successful reconstruction of the target state.



\subsection{Gradient Free Method: Evolutionary Strategy}

While gradient-based methods achieved fidelities approaching 1 in noiseless simulations, they required extensive manual tuning of both neural network hyperparameters and the optimization strategy. This issue became more severe in the presence of noise, where gradient signals were often unstable, making training less reliable and substantially increasing the number of epochs required for convergence. For higher-dimensional quantum states, the achievable fidelity typically plateaued around 0.85, falling short of the desired 0.99.

A significant contributor to the overall computational cost was the gradient estimation process. Since the SWAP test is inherently non-differentiable, we employed finite difference methods to approximate gradients with respect to each component of the generated state vector. This approach proved to be computationally intensive, as it necessitated a large number of quantum circuit executions per optimization step.

To address these limitations, we explored gradient-free optimization techniques such as Evolutionary Strategies (ES) \cite{salimans_evolution_2017} and Reinforcement Learning (RL). While RL failed to reliably converge to high-fidelity solutions, ES consistently outperformed gradient-based methods in both fidelity and convergence speed.


We introduce \textbf{QESwap (Quantum Evolutionary Strategy with SWAP Fidelity)}, a customized Evolutionary Strategy for reconstructing unknown quantum states using fidelity scores from the SWAP test. Unlike traditional gradient-based approaches, QESwap operates in a derivative-free regime, leveraging Gaussian perturbations and population-based search to iteratively maximize fidelity between a generated and unknown target state. Crucially, QESwap is designed for single-copy, non-destructive quantum learning — making it ideal for mid-circuit state reconstruction and dynamic memory applications. To our knowledge, this is the first ES framework to integrate SWAP-test-based fidelity estimation into a hybrid quantum-classical optimization loop.


Our method is implemented using \texttt{PennyLane} and \texttt{PyTorch}, integrating both classical and quantum components to iteratively optimize the representation of a target quantum state—be it a state vector, density matrix, or unitary matrix. 

Without loss of generality, we describe our approach using the state vector representation as follows.

\begin{algorithm}[H]\label{algo:QESwap}
\caption{QESwap: Evolutionary Strategy for Fidelity Optimization}
\begin{algorithmic}[1]
\State Initialize population size \( N \), noise scale \( \sigma \), learning rate \( \alpha \), and parameters \( \mathbf{w} \sim \mathcal{N}(0, I) \)
\For{each iteration up to max\_iter}
    \State Sample noise vectors \( \mathbf{z}_i \sim \mathcal{N}(0, I) \) for \( i = 1, \dots, N \)
    \State Generate candidates: \( \mathbf{w}_i = \mathbf{w} + \sigma \mathbf{z}_i \)
    \State Normalize \( \mathbf{w}_i \) and convert to \( |\psi_{\text{gen}}^{(i)}\rangle \)
    \State Evaluate fidelity \( F_i = \text{SWAPTest}( |\psi_{\text{gen}}^{(i)}\rangle, |\psi_{\text{unknown}}\rangle ) \)
    \State Compute advantages: \( A_i = \frac{F_i - \bar{F}}{\text{std}(F)} \)
    \State Update: \( \mathbf{w} \leftarrow \mathbf{w} + \frac{\alpha}{N \sigma} \sum_i A_i \mathbf{z}_i \)
    \If{fidelity exceeds threshold}
        \State \textbf{break}
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

\subsubsection{Problem Setup}

Let the unknown quantum state be denoted by \( |\phi_{\text{unknown}}\rangle \), a normalized complex-valued vector in a \( 2^n \)-dimensional Hilbert space for \( n \) qubits. The goal is to estimate a parametrized vector \( |\psi_{\text{gen}}(\mathbf{w})\rangle \) such that the fidelity 
\[
F = \left| \langle \phi_{\text{unknown}} \mid \psi_{\text{gen}}(\mathbf{w}) \rangle \right|^2
\]
is maximized. 

This optimization is performed using our proposed QESwap algorithm, with the swap test implemented as a quantum circuit to estimate fidelity. The SWAP test \ref{swap_test} is exactly the same as described in the gradient-based approach. 



\subsubsection{Evolutionary Strategy Optimization}

The ES algorithm searches for the optimal parameters \( \mathbf{w} \in \mathbb{R}^{2 \cdot 2^n} \), representing the real and imaginary parts of a candidate state. Each candidate state is parameterized as a vector \( \mathbf{w} \in \mathbb{R}^{2d} \), where \( d = 2^n \), with real and imaginary components flattened into a single vector. No assumptions are made about the structure or sparsity of the target state. The algorithm \ref{algo:QESwap} proceeds as follows:

\begin{itemize}
    \item Initialize \( \mathbf{w} \) with a Gaussian distribution.
    \item In each iteration, generate a population of \( N = 50 \) perturbed candidates using Gaussian noise.
    \item All candidate vectors \( \mathbf{w} \in \mathbb{R}^{2d} \) are interpreted as complex vectors by pairing consecutive entries as real and imaginary parts. Each candidate state \( |\psi_{\text{gen}}\rangle \) is normalized to unit norm before fidelity evaluation to ensure physical validity.

    \item Evaluate the swap test fidelity for each candidate.
    \item Compute the standardized rewards and update \( \mathbf{w} \) using:
    \[
    \mathbf{w} \leftarrow \mathbf{w} + \frac{\alpha}{N \sigma} \sum_i A_i \cdot \mathbf{z}_i,
    \]
    where \( \alpha = 0.05 \) is the learning rate, \( \sigma = 0.1 \) is the noise scale, \( A_i \) is the normalized advantage of the \( i \)-th candidate, and \( \mathbf{z}_i \) is its noise vector.
\end{itemize}

Training is terminated when either the maximum iteration count (100) is reached or when fidelity exceeds predefined thresholds (e.g., 0.95 or 0.99). All generated candidates are normalized before fidelity evaluation.

\subsubsection{Experimental Protocol}

We conduct experiments for 1 to 6-qubit systems. For each configuration, 1000 independent trials are performed with randomly sampled unknown quantum states. The QESwap algorithm is used to reconstruct each state, and the fidelity and convergence epoch for thresholds \( F \geq 0.95 \) and \( F \geq 0.99 \) are recorded.
 
All simulations are performed on noisy and noiseless quantum simulators and only single qubit results are performed in hardware as mentioned in \ref{tab:all_results}.
\subsection{Saving and Withdrawing the Quantum State}
% Once target unknown states are retrieved the complex-valued vectors are stored in classical memory using traditional methods. When queried using wither classical access technique or QRAM methods , the classical states are loaded using Stateprep methods. 
Once the target unknown states are retrieved, the corresponding complex-valued vectors are stored in classical memory using standard techniques. When queried—either through classical access methods or via QRAM—the stored states are reloaded into quantum circuits using state preparation routines.

==> todo.tex <==
%to do
1. Results for known states. 
2. Write explaining the figures in methods
% 5. SHow how generated states evolve over training iteration. Use Bloch sphere for demonstration. 
% 6. How much time is needed to reconstruct a state reliably? time vs reliability (with 1signma , 2 sigma etc. ) if the reconstruction time small enough to hold for decoherence time
% 7. How many copies are needed? How many shots reqd? relation to decoherence time
Per epoch time

# Add noisy bad results which shows noise affects 
